New Particles Working Group Report of the Snowmass 2013 Community Summer Study

This report summarizes the work of the Energy Frontier New Physics working group of the 2013 Community Summer Study (Snowmass).

==> NewParticles/story9-Aug05.tex <==
%\documentclass[11pt]{article}
%\usepackage{geometry}                % See geometry.pdf to learn the layout options. There are lots.
%\geometry{letterpaper}                   % ... or a4paper or a5paper or ... 
%%\geometry{landscape}                % Activate for for rotated page geometry
%%\usepackage[parfill]{parskip}    % Activate to begin paragraphs with an empty line rather than an indent
%\usepackage{graphicx}
%\usepackage{amssymb}
%\usepackage{epstopdf}
%\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}
%
%\title{An $A\to Zh$ bedtime story.}
%\author{Nathaniel Craig}
%\date{}                                           % Activate to display a given date or no date
%
%\begin{document}


% \subsection{Higgs Beyond the Standard Model}
The discovery of the 125~GeV Higgs boson has made a fundamental change in our view of
particle physics.
The properties of the Higgs already measured at the LHC are in agreement
with those of an elementary standard model Higgs boson at the $10\%$ level,
forcing the question of the naturalness of elementary scalars.
The naturalness of the Higgs boson requires new physics at the TeV
scale.
The observed Higgs particle may itself be the harbinger of new physics:
it may mix with other Higgs bosons in an extended Higgs sector,
have modified couplings due to standard model states,
or couple to new physics such as dark matter.
In this section we explore some of these possibilities.

\paragraph{Composite Higgs models:}
Besides supersymmetry, the other big idea for solving the naturalness
problem is compositeness of the Higgs sector.
This category includes models with extra dimensions at the TeV scale,
such as Randall-Sundrum models.
The most basic indication that the physics of extra dimensions is closely related 
to compositeness is that both predict towers of
resonances at the TeV scale.
This connection is a major theme of modern particle theory, extending
all the way from phenomenology and model-building to string theory
via the AdS/CFT correspondence.

%The most precise form of this equivalence is the duality between
%string theory in anti de Sitter space and supersymmetric gauge theory
%in $3+1$ dimensions (the AdS/CFT correspondence).
%This has played a large role in model-building, an unexpected 

After the discovery of the 125~GeV Higgs boson, the only natural version of
Higgs sector compositeness is that the observed Higgs boson is a
pseudo Nambu-Goldstone boson (PNGB) arising from
spontaneous breaking of a global symmetry at a scale above the TeV scale.
There are corrections to the couplings of the 125~GeV Higgs boson that are
proportional to $\xi = (v/f)^2$ where
$v = 246$~GeV is the vacuum expectation value of the Higgs boson and
$f$ is a compositeness scale.
The ratio $\xi$ is also a direct measure of the fine-tuning required in the 
model, and is presently required to be less than approximately $0.1$ due to
Higgs coupling measurements.
Improvements on Higgs coupling measurements will improve bounds on this 
parameter.

These PNGB Higgs models can be probed at hadron colliders in several ways.
First, additional naturalness considerations motivate the presence
of top partners in these models.
These can be searched for at hadron colliders, as discussed in 
\S\ref{sec:toppartners} below.
Second, the heavy resonances expected from the symmetry breaking sector
at the scale $f$ can be probed.
Limits from LHC run 1 for these particles require them to have masses above
2~TeV, and the LHC run 2 and HL-LHC will have additional reach for these
models.

At lepton colliders such as ILC and CLIC, the most sensitive probe
of the parameter $\xi$ is the Higgs coupling fit.
For example, these can reach down to $\xi \sim 0.002$
at 3~TeV CLIC with a luminosity of 1$/$ab \cite{clicwp,cliccdr}.
The impact of other future colliders for the Higgs coupling fit
is discussed in the Higgs working group report.
In addition, CLIC has a high sensitivity to enhanced double Higgs production,
which is a direct consequence of the compositeness of the Higgs
boson and therefore a `smoking gun' for composite modes.
This also directly measures the parameter $\xi$ and can be probed
down to $\xi = 0.03$ \cite{clicwp}.

%The reach for CLIC and other colliders is shown in Fig.~\ref{fig:compositeHiggs}.
%
%
%\begin{figure}
%\centering
%\includegraphics[width=0.4\linewidth]{NewParticles/figures_9/Composite_Higgs_CLIC}
%\caption{Bounds on composite Higgs models from LHC run 1 direct searches
%for vector resonances (brown region on the left), 
%precision Higgs coupling measurements (`LHC single Higgs'),
%and double Higgs production (`LHC double Higgs').
%These are compared with the sensitivity of 3~TeV CLIC with 1/ab for double
%Higgs production \cite{clicwp}.
%The region preferred from electroweak precision tests is the region
%below the line labelled `EWPT $\De\rho = 1.5 \times 10^{-3}$.}
%\label{fig:compositeHiggs}
%\end{figure}





\paragraph{Exotic Higgs decays:}
An essential component of the research program of the LHC, and any other 
future high-energy collider is the search for non-standard (`exotic') decays 
of the 125-GeV Higgs boson, {\it i.e.}~decays of a SM-like Higgs boson into 
one or more particles beyond the SM.
Non-standard Higgs decays have always been a well-motivated possibility as evidenced 
by an extensive existing, and growing, literature 
(see~\cite{exotics} for a comprehensive survey of the possibilities and 
an extensive list of references).
They remain a well-motivated possibility even with the discovery of a Higgs particle 
that is consistent with the simplest SM expectations, and they must be searched
for explicitly as they are often
unconstrained by other analyses.

The Higgs is the only SM particle that can have renormalizable couplings to 
SM gauge singlet fields.
This, together with the strikingly narrow width of the SM Higgs boson, 
implies that a small coupling of the Higgs to a new, 
light state can easily give rise to sizable branching ratios to non-standard decay modes.  For example, the addition of a singlet scalar field $S$ to the SM, which couples to 
the Higgs through a quartic interaction of the form
$\lambda S^2 H^2$ is a common building block in models of extended Higgs sectors.
Even a coupling as small as $\lambda = 5\times 10^{-3}$ yields a $10\%$ 
branching ratio of $h\to SS$ (for $m_S < m_h/2$).  
Exotic Higgs decays are a generic feature of extensions of the SM that contain light
states, and naturally arise in many models of electroweak symmetry breaking, 
such as the NMSSM and Little Higgs models. % , and 2 Higgs doublet models with a singlet.
A detailed experimental characterization of the Higgs boson at 
125~GeV includes searches for
{\it e.g.}~$h \to {\rm invisible}$, $(1,2)\gamma+{\rm MET}$, 
$\gamma+Z'$, $Z'+{\rm MET}$, lepton- or photon-jets, isolated leptons+MET, 
$4x, 2x2y$ (with $x, y = e, \mu, \tau$-leptons, MET, jets, or $b$-jets), 
with or without displaced vertices.



One of the best-motivated examples
of exotic Higgs decays is the decay of the 125~GeV Higgs to invisible
particles.
This is strongly motivated by the coupling of the Higgs to dark matter.
Indeed, such a coupling gives a direct detection cross section of the
size that is currently being probed in dark matter direct detection
experiments.

LHC limits on the branching ratio $h \to \mbox{invisible}$
are $0.65$ (ATLAS) \cite{ATLAS-CONF-2013-011} 
and $0.75$ (CMS) \cite{CMS-PAS-HIG-13-018}.
This illustrates that there is a great deal of room for new physics
in this channel.
The Snowmass Higgs working group concludes that the
LHC14 with 300/fb will probe branching fractions in the range
$0.17$--$0.28$, while the HL-LHC will probe branching
fractions in the range $0.06$--$0.17$.
The quoted ranges depend on the control of systematics.
Overall, the HL-LHC provides an order of magnitude improvement
in the reach for this mode.
The invisible decay of the Higgs can be cleanly studied at
$e^+ e^-$ colliders via $Zh$ production.
There are no studies for VLHC, but the LHC results
provide a proof of concept that this is possible.

Another example that has been studied for this report
is the cascade decay $h_1 \to aa \to (\tau\tau)(\tau\tau)$
at ILC \cite{Potter}.
This is a potential signal in the next-to-minimal SUSY standard model
(NMSSM).
This is an interesting example of an early discovery mode at a 250~GeV ILC.
Additionally, the masses can be measured to better than $1\%$ 
at this facility.


\paragraph{Connection with neutrino masses:}
A more speculative but very interesting possibility is that the Higgs
discovered at the LHC is part of an extended Higgs sector at the TeV
scale that also generates naturally small neutrino masses.
A very interesting example of this possibility is the type-II see-saw
model consisting of a Higgs triplet coupling to left-handed leptons
and the Higgs doublet.
This model contains a doubly-charged Higgs scalar with lepton number
violating decays to same-sign $ee$, $\mu\mu$, and $\tau\tau$.
Searches at LHC have placed limits of $m_{H^{++}} > 400$~GeV
using $4.7/$fb at 7 TeV \cite{ATLAS:2012hi}.
LHC run 2 can extend the reach for the charged Higgs to approximately
1~TeV in favorable cases.
The branching ratios to various charged lepton flavors are correlated
with the neutrino masses, so that the neutrino mass hieararchy can be
determined from collider data.
This provides an exciting connection with the neutrino physics program.
A well-motivated extension of this model is left-right symmetric model,
which contains a right-handed $W$ boson that can be observed at the
HL-LHC up to masses up to 4~TeV.




\paragraph{Extended Higgs sectors:}
Additional Higgs bosons are predicted by many well-motivated extensions of the 
Standard Model, including supersymmetry and some composite Higgs models. 
Searches for these states are also motivated simply from the need to
fully explore the Higgs sector.
Mixing between the 125~GeV Higgs and additional
Higgs bosons modifies the couplings of the observed
125~GeV Higgs compared to standard model values.
Therefore, searches for new Higgs states and precision Higgs coupling measurements
are complementary approaches to the important problem of studying the newly-found
Higgs particle.
We will discuss this in the context of a 2 Higgs doublet model (2HDM),
in which the observed 125~GeV state is the lightest CP-even neutral scalar $h$.
In addition, this model contains another neutral CP-even scalar $H$,
a CP-odd neutral scalar $A$, and a charged Higgs $H^\pm$.
In addition to the masses of the various Higgs bosons, the model
depends on the CP-even mixing angle $\alpha$ and the ratio of 
vacuum expectation values of the 2 Higgs doublets
$\tan\beta = v_1/v_2$.

The Higgs coupling constant fits for the 2HDM restrict the model
to small values of $\cos(\beta - \alpha)$.
This is naturally realized in the decoupling limit where one
linear combination of the Higgs doublets is getting heavy.
Direct searches for new Higgs bosons can probe closer to
$\cos(\beta - \alpha)$ if the masses of these states are sufficiently
light, making these approaches complementary.



Higgs bosons generally couple most strongly to particles with the largest mass, 
motivating  searches for new particles that decay to vector bosons, 
the $h^0$, or heavy fermions (top/bottom/tau). 
These couplings also lead to appreciable production rates at both hadron and lepton 
colliders. 

At hadron colliders, two senstive searches are
$H \to ZZ \to 4\ell$ and $A \to Zh$ followed by $Z \to \ell\ell$
and $h \to bb$ or $\tau\tau$.
The reach for the first signal is given for the 14 TeV LHC in
Fig.~\ref{fig:HZZreach}, and the second in Fig.~\ref{fig:AZhreach}.




\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{NewParticles/figures_9/HZZ_300_5sigma}
\caption{$5\sigma$ discovery reach for 300~GeV $H$ 
decaying via $H \rightarrow ZZ \rightarrow 4\ell$.
Blue (green) region is for LHC14
with 300$/$fb (3000$/$fb) \cite{2HDMwp}.
The star denotes the parameter point used in the discovery story below.
{\bf [should be at $\tan\beta = 2$]}}
\label{fig:HZZreach}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{NewParticles/figures_9/AZh_300_5sigma}
\caption{$5\sigma$ discovery reach for 300~GeV $A$ 
decaying via $A \rightarrow Z h^0 \rightarrow (\ell\ell)(bb
\mbox{ or } \tau\tau$.
Blue (green) region is for LHC14
with 300$/$fb (3000$/$fb) \cite{2HDMwp}.
The star denotes the parameter point used in the discovery story below.
{\bf [should be at $\tan\beta = 2$]}}
\label{fig:AZhreach}
\end{figure}


At hadron colliders, the $H$ and $A$ can be copiously singly
produced through gluon fusion or $b \bar b$ and $t \bar t$ 
associated production. 
Charged Higgs bosons can be produced singly via $t b$ associated production 
at $pp$ colliders 
or pair-produced via Drell-Yan processes at $e^+ e^-$ colliders. 
Decays of these additional states may be observed in standard Higgs search channels or novel
resonant channels involving the 125~GeV Higgs such as $Wh, Zh,$ or $hh$.

At $e^+ e^-$ colliders,
for a wide range of models
$H^+ H^-$ and $H A$ can be observed as long as the sum of the masses
is below the center of mass energy of the collider.
Furthermore, the masses of the observed states
can be measured to better than $1\%$ \cite{clicwp}.
Consequently, CLIC is ideally suited for the study of Higgs bosons
with masses up to $1.5$~TeV.



%An extended Higgs sector provides extensive opportunities for interplay between coupling 
%measurement of the 125~GeV Higgs and direct searches for new states. 
%In general, the presence of additional Higgs bosons implies that the 125~GeV Higgs is not 
%completely aligned with the vacuum expectation value (VEV) that breaks electroweak symmetry, 
%giving rise to deviations from Standard Model Higgs couplings. 
%At one extreme, these deviations may be large enough for precision Higgs coupling 
%measurements  to provide the first indication of an extended Higgs sector. 
%Alternately, the 125~GeV Higgs may be closely aligned with the symmetry-breaking VEV, 
%in which case deviations in observed Higgs couplings are small but additional Higgs scalars 
%retain couplings to Standard Model fermions and may still be copiously produced at colliders. 
%In the event of positive signals in any search channel, the combination of direct searches 
%and coupling measurements allow powerful discrimination between possible models. 



In the scenario we now discuss, 
we consider a signal at LHC14/300 for $A \to Zh \to (bb)(\ell\ell)$.
There is significant reach for discovery in this channel, as can be seen in
Fig.~\ref{fig:AZhreach}.
For this scenario, we assume a type-II 2HDM with $m_A = 325$~GeV,
and $\alpha = -0.475$, $\tan \beta = 2$.


By the end of the 14 TeV run with 300 fb$^{-1}$ of integrated luminosity, an excess is 
observed in searches for anomalous $Zh$ production in the $bb \ell \ell$ final state consistent with a production cross section times branching ratio of $\sim 10$~fb. 
The full $m_{\ell \ell b b}$ invariant mass distribution peaks around 325 GeV. 
The lepton pair production is consistent with the leptonic decay of a $Z$ boson, 
while the invariant mass of the bottom quark pair is consistent with the decays of the observed SM-like Higgs boson at 125 GeV. 
The signal significance is $\sim 2.5 \sigma$. 
There is also a mild $\sim 1 \sigma$ excess in the $\tau^+ \tau^- \ell \ell$ channel 
where the lepton pairs are again consistent with leptonic decay of a $Z$ boson, 
but without sufficient mass resolution to conclusively relate to the excess in the 
$bb \ell \ell$ final state. 
The final states and approximate mass reconstruction in the $bb \ell \ell$  
final state  are consistent with the production of a pseudoscalar Higgs boson with 
decay to $Zh$. 

At the same time, there are no meaningful excesses in searches for resonant $WW$ and 
$ZZ$ di-boson production in this mass range, nor are there any meaningful signals 
in the ongoing searches for additional MSSM Higgs bosons in the $bb$ and $\tau \tau$ 
final states at large $\tan \beta$.  
In the context of a two-Higgs-doublet model, the natural interpretation is the 
CP-odd pseudoscalar $A$ at low $\tan \beta$, where the branching ratio for $A \to Zh$ 
may be appreciable but the rates for gluon fusion or $bbA$ associated production with 
$A \to bb, \tau \tau$ are not large enough to be distinguished from background. 


Motivated by these excesses, a search conducted in the 300 fb$^{-1}$ data set for 
$\ell \ell + \gamma \gamma$ consistent with anomalous $Zh$ production yields 
$\sim 3$ events whose $m_{\ell \ell \gamma \gamma}$ accumulate at 325 GeV, 
further suggesting the presence of a new state decaying to $Zh$ but not 
substantially increasing the significance of the excess. 
Given that these signals in the $Zh$ final state are consistent with a pseudoscalar 
Higgs at low $\tan \beta$, both collaborations consequently extend their inclusive 
diphoton resonance searches to close the gap in coverage between the endpoint of the 
SM-like Higgs search at 150 GeV and the beginning of the KK resonance search at 500 GeV. 
Upon unblinding the analysis, they detect a signal consistent with the production and 
decay of a 325 GeV particle decaying to pairs of photons with 
$\sigma \cdot {\rm Br} \sim 7$ fb at 14 TeV. 
The lack of events in dijet-tagged categories indicate that there is no meaningful 
associated production, bolstering the case for a new pseudoscalar.


Attempts to interpret the resonance in terms of the MSSM are stymied by the resolution 
of Higgs coupling measurements in the 300 fb$^{-1}$ data set. 
For a pseudoscalar in the MSSM at low $\tan \beta$ with $m_A = 325$ GeV, the generic 
expected deviation in the $hbb$ coupling is of order $\sim 5-20\%$, with much smaller 
deviations in $h \gamma \gamma$, $htt$, and $hVV$. 
The precision of Higgs coupling measurements at 300 fb$^{-1}$ only serve to bound 
$\tan \beta < 4$ in the MSSM. Both the high-luminosity run of the LHC and the 
ILC become high priorities for establishing the discovery of the new state and 
triangulating measurements of Higgs couplings at both 125 GeV and 325 GeV.
 
At the high luminosity run of the LHC, the signal reaches $5 \sigma$ significance in the $bb \ell \ell$ final state by 1000 fb$^{-1}$ of integrated luminosity, sufficient to announce the discovery of a new state. The excess in the $\tau^+ \tau^- \ell \ell$ channel grows to several $\sigma$, consistent with a production cross section times branching ratio of $\sim 1$ fb, while the excess in the diphoton final state at 325 GeV also reaches $5 \sigma$ significance by the end of the full 3000 fb$^{-1}$. However, the experimental and theoretical errors on the discovery-level channels are sufficiently large that interpretation based on direct coupling measurements of the new state remains challenging. Interpreted in the context of a Type II 2HDM, the best fit to the production and decay rates favors $\tan \beta \simeq 2, \cos (\beta - \alpha) \simeq -0.012$. This is in mild tension with the MSSM interpretation, for which the tree-level prediction at $\tan \beta \simeq 2$ is closer to $\cos (\beta - \alpha) \simeq -0.04$, but without sufficient experimental resolution to provide meaningful discrimination. Although the errors on the Higgs coupling measurements at 125 GeV improve to $\Delta g_{hbb} \sim 10\%$, still no significant deviation from Standard Model predictions is observed. Finally, after the full 3000 fb$^{-1}$ are analyzed, a collection of 10 $4\ell$ events consistent with $H \to ZZ \to 4 \ell$ are reconstructed around 450 GeV -- sufficient to hint at the presence of an additional CP-even scalar but insufficient to establish discovery. Searches for a resonance in $t \bar t$ prove inconclusive.

A lepton collider such as the ILC or TLEP can explore the electroweak symmetry breaking
sector in detail.
For example,
at the $\sqrt{s} = 250$ GeV run of an ILC, the coupling measurements of the 125 GeV Higgs improve to $\Delta g_{hbb} \sim 5\%$ without observing deviations from SM predictions, increasing tension with the MSSM interpretation. No direct production of the new state is kinematically possible. However, at $\sqrt{s} = 500$ GeV, the pseudoscalar is expected to be kinematically available in both $b \bar b A$ and $Ah$ associated production. 
Indeed, after 500 fb$^{-1}$ are on tape, $b \bar b A$ associated production is observed 
at the level of a small handful of events consistent with $\sigma(b \bar b A) \sim 0.1$ fb. 
Two $Zhh$ events are observed consistent with $e^+ e^- \to Ah \to Zhh,$ but are difficult to distinguish from the SM di-Higgs background given the low statistics. 
By $\sqrt{s} = 1$ TeV the $bbA$ signal increases consistent with a cross section of 
$\sim 1$ fb, leaving several hundred $b \bar b A$ events on tape and substantially 
improving the direct coupling measurements of the pseudoscalar. Most importantly, the ILC operating at $\sqrt{s} = 1$ TeV discovers additional states in the Higgs sector. The first is a 370 GeV charged Higgs with cross section of order $\sim 10$ fb. The primary discovery mode is $H^+ H^-$ Drell-Yan pair production in the $t \bar t b \bar b$ final state. The mass splitting between the charged Higgs and the pseudoscalar are again in tension with tree-level MSSM predictions for the mass spectrum. Reaching closer to the kinematic threshold, the ILC discovers the hinted-at CP-even scalar at 450 GeV through $HA$ associated production in the final state $t \bar t Z h$ with a cross section of several femtobarn. 

In addition, the improvement of Higgs coupling measurements at 125 GeV indicates 
a small persistent tension with SM predictions at the level of $\Delta g_{hbb} \sim 2\%$.
While the departure is not statistically significant, the smallness of $\Delta g_{hbb}$ 
is in tension with conventional MSSM predictions. 
In the context of a Type II 2HDM, the combination of measurements of the light SM-like Higgs at 125 GeV, the pseudoscalar at 325 GeV, the charged Higgs at 370 GeV, and the second CP-even scalar at 450 GeV imply an extended Higgs sector that is closer 
to the alignment limit than implied by supersymmetric decoupling alone, with the best-fit point in a Type II 2HDM ultimately corresponding to $\tan \beta = 2, \cos (\beta - \alpha) = -0.0122$, as well as with mass relations between scalars that are discrepant from the standard MSSM predictions. This ignites fervent exploration of non-standard corners of MSSM Higgs parameter space, 
as well as  other natural theories of extended electroweak symmetry breaking. 

A high-energy proton collider can also continue exploration of the extended Higgs sector by producing a large sample of heavier Higgs scalars. In this example, although the heavy CP-even scalar $H$ primarily decays to $t \bar t$ pairs, it also exhibits rarer decay modes such as $H \to ZA$ and $H \to H^\pm W^\mp$ that are kinematically squeezed but nonetheless observable provided the large number of $H$ bosons produced at a high-energy $pp$ machine. More generally, a high-energy proton collider has the potential to discover additional Higgs bosons that lie well beyond the reach of the LHC and ILC.



%\end{document}  


==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

